A Lightweight Moving Target Defense Framework for Multi-purpose Malware Affecting IoT Devices

Malware affecting Internet of Things (IoT) devices is rapidly growing due to the relevance of this paradigm in real-world scenarios. Specialized literature has also detected a trend towards multi-purpose malware able to execute different malicious actions such as remote control, data leakage, encryption, or code hiding, among others. Protecting IoT devices against this kind of malware is challenging due to their well-known vulnerabilities and limitation in terms of CPU, memory, and storage. To improve it, the moving target defense (MTD) paradigm was proposed a decade ago and has shown promising results, but there is a lack of IoT MTD solutions dealing with multi-purpose malware. Thus, this work proposes four MTD mechanisms changing IoT devices' network, data, and runtime environment to mitigate multi-purpose malware. Furthermore, it presents a lightweight and IoT-oriented MTD framework to decide what, when, and how the MTD mechanisms are deployed. Finally, the efficiency and effectiveness of the framework and MTD mechanisms are evaluated in a real-world scenario with one IoT spectrum sensor affected by multi-purpose malware.

==> Figure-Ransomware-Validation.tex <==

\begin{figure}[H]
\begin{tikzpicture}
\begin{axis}[
    xlabel={Time [s]},
    ylabel={System Resource Usage [\%]},
    xmin=200, xmax=500,
    ymin=0, ymax=130,
    xtick={250, 350, 450},
    ytick={0, 25, 50, 75, 100},
    legend pos=north east,
    width=\linewidth,
    legend cell align={left},
    height=4.8cm,
    ymajorgrids=true,
    grid style=dashed,
]

\addplot[
    ]
    coordinates {
    (0,25)(14,17)(28,25)(42,23)(56,21)(70,21)(84,18)(98,23)(112,23)(126,25)(140,14)(154,18)(168,25)(182,19)(196,19)(210,23)(224,26)(238,19)(252,43)(266,94)(280,93)(294,76)(308,84)(322,75)(336,79)(350,76)(364,75)(378,50)(392,27)(406,23)(420,25)(434,21)(448,23)(462,26)(476,22)(490,24)(504,21)(518,21)(532,23)(546,25)(560,24)(574,21)(588,23)(602,24)(616,28)(630,20)(644,16)(658,22)(672,28)(686,16)(700,17)(714,24)(728,22)(742,20)(756,24)(770,25)(784,24)(798,17)(812,22)(826,23)(840,29)(854,21)(868,20)(882,26)(896,19)(910,25)(924,29)(938,26)(952,24)(966,27)(980,25)(994,19)(1008,18)(1022,23)(1036,19)
    };
    \addlegendentry{CPU}
    
\addplot[
    legend style={at={(0.02,0.02)},anchor=south west},
    color=black,
    dashed
    ]
    coordinates {
    (0,9.37303899310746)(14,9.38946681019749)(28,9.37099827048758)(42,9.38446703977879)(56,9.51599161263003)(70,9.45364753659271)(84,9.44334188736232)(98,9.44436224867225)(112,9.44436224867225)(126,9.45395364498569)(140,9.45130070557985)(154,9.44650500742313)(168,9.44956609135295)(182,9.45558622308159)(196,9.46997331755175)(210,9.5131346009622)(224,9.51395089001015)(238,9.53027667096919)(252,9.62986393481932)(266,9.84036447305991)(280,9.89556601992766)(294,9.89668841736859)(308,9.91556510160248)(322,9.96199154120474)(336,9.81689616293129)(350,9.81618191001434)(364,9.81546765709738)(378,9.80720273048687)(392,9.63588406654796)(406,9.62241529725676)(420,9.62302751404272)(434,9.63231280196318)(448,9.62996597095031)(462,9.59200853022055)(476,9.62578248957956)(490,9.62221122499477)(504,9.60772209439363)(518,9.61904810493396)(532,9.62282344178073)(546,9.6165992377901)(560,9.61966032171992)(574,9.62568045344857)(588,9.61221168415736)(602,9.61884403267197)(616,9.6115994673714)(630,9.61843588814799)(644,9.61251779255034)(658,9.62149697207781)(672,9.61731349070706)(686,9.60496711885679)(700,9.59211056635155)(714,9.59374314444745)(728,9.59935513165212)(742,9.58343749521706)(756,9.5910902050416)(770,9.61476258743221)(784,9.60068160135504)(798,9.60047752909305)(812,9.61976235785092)(826,9.60588544403573)(840,9.60792616665561)(854,9.60088567361703)(868,9.5996612400451)(882,9.61976235785092)(896,9.60690580534567)(910,9.60751802213164)(924,9.60915060022754)(938,9.60353861302287)(952,9.60119178201001)(966,9.60945670862052)(980,9.58935559081471)(994,9.5997632761761)(1008,9.5860904346229)(1022,9.61904810493396)(1036,9.61068114219245)
    };
    \addlegendentry{RAM}
    
\addplot[
    legend style={at={(0.02,0.02)},anchor=south west},
    color=black,
    mark=square
    ]
    coordinates {
    (0,0)(14,0)(28,0)(42,0)(56,0)(70,0.17574692442882248)(84,0)(98,0)(112,0)(126,0)(140,0)(154,0)(168,0)(182,0)(196,0)(210,0)(224,0)(238,0)(252,0)(266,0.4393673110720563)(280,0)(294,0)(308,18.36555360281195)(322,5.623901581722319)(336,0)(350,0)(364,0)(378,0)(392,0)(406,0)(420,0)(434,0)(448,0)(462,0)(476,0)(490,0)(504,0)(518,0)(532,0)(546,0)(560,0)(574,0)(588,0)(602,0)(616,0)(630,0)(644,0)(658,0)(672,0)(686,0)(700,0)(714,0)(728,0)(742,0)(756,0)(770,0)(784,0)(798,0)(812,0)(826,0)(840,0)(854,0)(868,0)(882,0)(896,0)(910,0)(924,0)(938,0)(952,0)(966,0)(980,0)(994,0)(1008,0)(1022,0)(1036,0)(1050,0)
    };
    \addlegendentry{Disk Read}
    
\addplot[
    legend style={at={(0.02,0.02)},anchor=south west},
    color=black,
    mark=triangle,
    ]
    coordinates {
    (0,0.4959159859976663)(14,0)(28,0.10210035005834306)(42,0.05834305717619603)(56,0.1750291715285881)(70,0)(84,0)(98,0.08751458576429405)(112,0)(126,0)(140,0)(154,0)(168,0)(182,0)(196,0)(210,0)(224,0.08751458576429405)(238,0.043757292882147025)(252,0)(266,0.1750291715285881)(280,0.1896149358226371)(294,12.310385064177364)(308,0)(322,0)(336,16.525670945157525)(350,0.043757292882147025)(364,0)(378,0)(392,0)(406,0)(420,0)(434,0)(448,0)(462,0)(476,0)(490,0)(504,0)(518,0)(532,0)(546,0)(560,0)(574,0)(588,0)(602,0)(616,0)(630,0)(644,0)(658,0)(672,0)(686,0)(700,0)(714,0)(728,0)(742,0)(756,0)(770,0)(784,0)(798,0)(812,0)(826,0)(840,0)(854,0)(868,0)(882,0)(896,0)(910,0)(924,0)(938,0)(952,0)(966,0)(980,0)(994,0)(1008,0)(1022,0)(1036,0)(1050,0)
    };
    \addlegendentry{Disk Write}
    
   \draw[blue] (axis cs: 251,0) -- 
       (axis cs: 251,85)node[anchor=center, above=0.5pt]{\small{(1)}};
   \draw[blue] (axis cs: 265,0) -- 
       (axis cs: 265,105)node[anchor=center, above=0.5pt]{\small{(2)}};
   \draw[blue] (axis cs: 341,0) -- 
       (axis cs: 341,100)node[anchor=center, above=0.5pt]{\small{(3)}};
    
    
\end{axis}
\end{tikzpicture}
\caption{Device Resource Impact of Mitigating Ransomware}
\label{fig:ransomware}
\end{figure}




